There Are a Thousand Hamlets in a Thousand People's Eyes: Enhancing Knowledge-grounded Dialogue with Personal Memory

Knowledge-grounded conversation (KGC) shows great potential in building an engaging and knowledgeable chatbot, and knowledge selection is a key ingredient in it. However, previous methods for knowledge selection only concentrate on the relevance between knowledge and dialogue context, ignoring the fact that age, hobby, education and life experience of an interlocutor have a major effect on his or her personal preference over external knowledge. Without taking the personalization issue into account, it is difficult to select the proper knowledge and generate persona-consistent responses. In this work, we introduce personal memory into knowledge selection in KGC to address the personalization issue. We propose a variational method to model the underlying relationship between one's personal memory and his or her selection of knowledge, and devise a learning scheme in which the forward mapping from personal memory to knowledge and its inverse mapping is included in a closed loop so that they could teach each other. Experiment results show that our method outperforms existing KGC methods significantly on both automatic evaluation and human evaluation.

==> comment.tex <==
Dear Senior Area Chair:

We are grateful to all the reviewers for their time and effort spent on reviewing our manuscript. We carefully read their insightful comments one by one. We are glad that the novelty of our work and the efficacy of the proposed method are well acknowledged by the reviewers. 

Some shows interest in the newly-released dataset. The dataset, as well as the the code for crawling and processing the corpus will be made public to facilitate relevant research in the future. The final version will include a more detailed illustration about the dataset collection. We will provide several examples in appendix to help our readers have a better understanding. Besides, the typos and ambiguities will be revised following the suggestions of the reviewers.

Many thanks again for the program committees, area chairs and senior area chairs participated in the review process. 



==> explanatory.tex <==
Dear Ethics Chairs:

Thanks for your time and efforts in reviewing our work and your suggestions are of great significance to our work, which undoubtedly helps to improve our manuscript. 

We carefully read the ethics meta-review. Following your advice, we include ethical considerations as an independent section after the conclusion. In this section, we give an answer to your questions to the best of our knowledge. We sincerely hope it addresses your concerns properly. Besides, we are willing to make any additional revisions to meet the requirements of ACL 2022 conference at any time.

Best regards,
The authors of Paper998.

==> metalist.tex <==
1. The paper presentation could benefit from a rewriting that focuses on introducing the problem of personalized KGC and motivating it.

2. Authors should also discuss why it’s not enough to treat personal memory as just some additional knowledge candidates.

3. The corpus creation described in section 4.1 does not give enough details to understand exactly how knowledge and memory candidates are created. Authors should also give examples of the data that was collected.

4. The distillation process of closing the loop in the dual learning setup should be discussed in more detail. E.g., where is the equation 17 used in Algorithm 1?

5. The definition of personal memory was ambiguous and not fully defined. For instance, does this concept include false beliefs (incorrect knowledge), subjective opinions (unsupported knowledge) or inferential knowledge? What would be the unit of personal memory in the context of visually grounded dialogues (line 134)? How can we extend the idea to inter-personal knowledge, i.e. common ground?

6. More information/explanation concerning the collected dataset should be included (e.g. data collecting procedure and reviewing process).

7. In general, the writing quality seems weaker in the latter part of the paper (from the experimental results onward). Revising this section could benefit the overall clarity of findings and subsequent takeaway points.

8. Some aspects of the dataset are unclear. For instance: (a) following ACL ethics guidelines, was approval granted by an external institutional review board to collect and publish this data?; (b) what other requirements are there for data release (e.g., will a public link be provided, or will the data be available upon request from the authors)?; (c) how many annotators labeled each sample (and how many annotators were there in total)?; and (d) were all samples in English?

9. Some results seem very close, particularly in the ablation study. It is unclear whether the results in Table 5, for example, are statistically significant; if not, it may be good to temper the claims made based on these findings.
